Design of Classes I

The use of functional programming languages in the first programming course at many universities is well-established and effective. Invariably, however, students must progress to study object-oriented programming. This article presents how the first steps of this transition have been successfully implemented at Seton Hall University. The developed methodology builds on the students' experience with type-based design acquired in their previous introduction to programming courses. The transition is made smooth by explicitly showing students that the design lessons they have internalized are relevant in object-oriented programming. This allows for new abstractions offered by object-oriented programming languages to be more easily taught and used by students. Empirical evidence collected from students in the course suggests that the approach developed is effective and that the transition is smooth.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{P. Achten \& E. Machkasova  (Eds.): Trends in\\
Functional Programming in Education (TFPIE) 2021/22
\\
EPTCS 363, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.363.1}{10.4204/EPTCS.363.1}}
\pdfoutput=1

